On the Stability of Type II Blowup for the Keller-Segel System in High Dimensions

We study finite-time blowup for the parabolic--elliptic Keller--Segel system on $\mathbb{R}^d$ in dimensions $d\geq11$, where the problem is mass supercritical. For every integer $l\geq2$, we construct smooth radially symmetric solutions whose radial mass variable concentrates the normalized stationary state $Q$ at a quantized scale. Each blowup regime can be realized by solutions with nonnegative population density throughout their classical lifespan. More precisely, near the blowup time $T$, \[ u(t,r)=\frac{1}{\lambda^2(t)}\left[Q\left(\frac{r}{\lambda(t)}\right) +\epsilon\left(t,\frac{r}{\lambda(t)}\right)\right], \qquad \lambda(t)=c(T-t)^{\frac{l}{\gamma(d)}}(1+o(1)), \] where $c>0$ and $\gamma(d)=\frac12\bigl(d-2-\sqrt{(d-2)(d-10)}\bigr)$. The remainder $\epsilon$ converges to zero in local $L^\infty$ norms and in a range of high-order homogeneous Sobolev norms. Since $2l>\gamma(d)$, the concentration scale is strictly smaller than the parabolic scale $\sqrt{T-t}$, and the resulting blowup is of type II. The $l$-th regime has exactly $l-1$ unstable radial modulation directions and is stable within a codimension-$(l-1)$ class of suitably regular radial initial data. The proof combines a generalized-kernel expansion driven by the algebraic tail of $Q$, modulation analysis, coercive weighted high-order energy estimates, and a finite-dimensional topological argument. This yields a quantized hierarchy of stationary-state concentration rates for the high-dimensional Keller--Segel flow.

==> macro-3.tex <==
%!TEX root = products_of_random_matrices-v2.tex
%=================================================
% Packages
%=================================================

\synctex=1

%\usepackage{fixltx2e} % Makes \( \) equation style robust, among other
                      % things. Must be first package

\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{fancyhdr}
\usepackage{amsmath,amsfonts,amsbsy,amsgen,amscd,amssymb,amsthm}
%\usepackage{bbm}  % Loads too many fonts :(
%\usepackage{subfig}
\usepackage{url}

\usepackage{mathtools}

%\mathtoolsset{showonlyrefs}

\usepackage[font=small,margin=0.25in,labelfont={bf},labelsep={colon}]{caption}
%labelsep={space}

\usepackage{subcaption}

\usepackage{tikz}
\usepackage{microtype}
\usepackage{enumitem}

\definecolor{dark-gray}{gray}{0.3}
\definecolor{dkgray}{rgb}{.4,.4,.4}
\definecolor{dkblue}{rgb}{0,0,.5}
\definecolor{medblue}{rgb}{0,0,.75}
\definecolor{rust}{rgb}{0.5,0.1,0.1}

\usepackage[colorlinks=true]{hyperref}


\hypersetup{urlcolor=rust}
\hypersetup{citecolor=dkblue}
\hypersetup{linkcolor=dkblue}
%\hypersetup{linkcolor=black}

\usepackage{setspace}
%\doublespace

\usepackage{graphicx}
\usepackage{booktabs,longtable,tabu} % Nice tables
\setlength{\tabulinesep}{1mm}
\usepackage{multirow} % More control over tables

\usepackage{float}


\usepackage[full]{textcomp}

\usepackage[scaled=.98,sups,osf]{XCharter}% lining figures in math, osf in text
\usepackage[scaled=1.04,varqu,varl]{inconsolata}% inconsolata typewriter
\usepackage[type1]{cabin}% sans serif
\usepackage[charter,vvarbb,scaled=1.07]{newtxmath}
\usepackage[cal=boondoxo]{mathalfa}
\linespread{1.04}

\usepackage[T1]{fontenc}

%\usepackage{textcomp}
%     \usepackage[osf,scaled=.95]{heuristica} % osf for text, not math
%     \usepackage{cabin} % sans serif
%     \usepackage[varqu,varl]{inconsolata} % sans serif typewriter
%     \usepackage[utopia,bigdelims,vvarbb]{newtxmath} % bb from STIX
%     \usepackage[cal=boondoxo]{mathalfa} % mathcal

%
%\usepackage{fourier}
%\usepackage{charter}

%\usepackage[sc]{mathpazo}
%\usepackage{tgpagella}
%\linespread{1.05}

%\usepackage{tgpagella}

%\usepackage{kmath,kerkis}

%\usepackage[garamond]{mathdesign}
%\usepackage[charter]{mathdesign}
%\usepackage{fourier}
%\usepackage{times}

%\usepackage{garamondx}
%\usepackage[garamondx,cmbraces]{newtxmath}

%\newcommand\hmmax{0} % Default is 3.
%\newcommand\bmmax{0} % Default is 4.

\usepackage{bm} % boldmath must be called after the package


\graphicspath{{figures/}}

%=================================================
% Formatting
%=================================================

%\sloppy % Helps with margin justification

% \theoremstyle{theorem}

\newtheorem{bigthm}{Theorem}
\renewcommand{\thebigthm}{\Roman{bigthm}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{sublemma}[theorem]{Sublemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{result}[theorem]{Result}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}

\theoremstyle{definition}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}

%\newenvironment{example}[1][]{% 
%  \refstepcounter{theorem}%
%  \smallskip\par\textsc{Example~\thetheorem}. \textit{#1.}}%
%{\smallskip\par}
%\newenvironment{remark}{\stepcounter{theorem}\par\textit{Remark~\thetheorem.}}{\par}


\newenvironment{mainthm}{\par\textsc{Main theorem.}\it}{\par}


%%% Further font changes
\newcommand{\lang}{\textit}
\newcommand{\titl}{\textsl}
\newcommand{\term}{\emph}

%%% Equation numbering
\numberwithin{equation}{section} 
\numberwithin{figure}{section}
\numberwithin{table}{section}

\floatstyle{plaintop}
\newfloat{recipe}{thp}{lor}
\floatname{recipe}{Recipe}
\numberwithin{recipe}{section}

%%% Typesetting
\providecommand{\mathbold}[1]{\bm{#1}}  % Must be after 'fourier'

\allowdisplaybreaks[4]
                                % package loads
                                
\newcommand{\qtq}[1]{\quad\text{#1}\quad} % "Quad-Text-Quad"
                                
                                
%%% Annotations
\newcommand{\notate}[1]{\textcolor{red}{\textbf{[#1]}}}

%=================================================
% Symbols
%=================================================

%%% Old symbols with new names
\newcommand{\oldphi}{\phi}
\renewcommand{\phi}{\varphi}

\newcommand{\eps}{\varepsilon}

\newcommand{\oldmid}{\mid}
\renewcommand{\mid}{\mathrel{\mathop{:}}} 

%%% New symbols
\newcommand{\defby}{\overset{\mathrm{\scriptscriptstyle{def}}}{=}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\third}{\tfrac{1}{3}}

\newcommand{\sumnl}{\sum\nolimits}
\newcommand{\suml}{\sum\limits}

\newcommand{\defeq}{\ensuremath{\mathrel{\mathop{:}}=}} % Definition-equals
\newcommand{\eqdef}{\ensuremath{=\mathrel{\mathop{:}}}} % Equals-definition

%%% Constants
\newcommand{\cnst}[1]{\mathrm{#1}} 
\newcommand{\econst}{\mathrm{e}}
\newcommand{\iunit}{\mathrm{i}}

\newcommand{\onevct}{\mathbf{e}} % All ones vector
\newcommand{\zerovct}{\vct{0}} % Zero vector

\newcommand{\Id}{\mathbf{I}}
\newcommand{\onemtx}{\bm{1}}
\newcommand{\zeromtx}{\bm{0}}

%%% Sets
\newcommand{\coll}[1]{\mathscr{#1}}
\newcommand{\sphere}[1]{\mathsf{S}^{#1}}
\newcommand{\ball}[1]{\mathsf{B}^{#1}}
\newcommand{\Grass}[2]{\mathsf{G}^{#1}_{#2}}
\providecommand{\mathbbm}{\mathbb} % In case we don't load bbm
\newcommand{\Rplus}{\mathbbm{R}_{+}}
\newcommand{\R}{\mathbbm{R}}
\newcommand{\F}{\mathbbm{F}}
\newcommand{\C}{\mathbbm{C}}
\newcommand{\N}{\mathbbm{N}}
\newcommand{\Z}{\mathbbm{Z}}
\newcommand{\M}{\mathbbm{M}}

% Set operations
\newcommand{\polar}{\circ}
\newcommand{\closure}{\overline}
\newcommand{\bdy}{\mathrm{bdy}}

%%% Real and complex analysis
\newcommand{\abs}[1]{\left\vert {#1} \right\vert}
\newcommand{\abssq}[1]{{\abs{#1}}^2}

\newcommand{\sgn}[1]{\operatorname{sgn}{#1}}
\newcommand{\real}{\operatorname{Re}}
\newcommand{\imag}{\operatorname{Im}}
\newcommand{\pos}{\operatorname{Pos}}
\newcommand{\shrink}{\operatorname{Shrink}}

\newcommand{\diff}[1]{\mathrm{d}{#1}}
\newcommand{\idiff}[1]{\, \diff{#1}}


\newcommand{\grad}{\nabla} % Conflicts w/SIAM styles?
\newcommand{\subdiff}{\partial}

\newcommand{\argmin}{\operatorname*{arg\; min}}
\newcommand{\argmax}{\operatorname*{arg\; max}}

%%% Probability & measure

\newcommand{\Prob}[1]{\mathbbm{P}\left\{{#1}\right\}}
\newcommand{\Probe}[1]{\Prob\left({#1}\right)}
\newcommand{\Expect}{\operatorname{\mathbbm{E}}}

\newcommand{\normal}{\textsc{normal}}
\newcommand{\erf}{\operatorname{erf}}

\DeclareMathOperator{\rvol}{rvol}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\mVar}{\mathbold{\mathrm{Var}}}

\newcommand{\chisq}{\chi^2}

\newcommand{\Beta}{\mathrm{B}}


%%% Vector and matrix operators
\newcommand{\vct}[1]{\mathbold{#1}}
\newcommand{\mtx}[1]{\mathbold{#1}}
\newcommand{\Eye}{\mathbf{I}}

\newcommand{\trsp}{\mathsf{T}}
\newcommand{\adj}{*}
\newcommand{\psinv}{\dagger}

\newcommand{\lspan}[1]{\operatorname{span}{#1}}

\newcommand{\range}{\operatorname{range}}
\newcommand{\colspan}{\operatorname{colspan}}

%\newcommand{\rank}{\operatorname{rank}}
\newcommand{\nullity}{\operatorname{null}}

%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\ntr}{\operatorname{\bar{\trace}}}

%\newcommand{\supp}[1]{\operatorname{supp}(#1)}

\newcommand{\smax}{\sigma_{\max}}
\newcommand{\smin}{\sigma_{\min}}

\newcommand{\nnz}{\operatorname{nnz}}
\renewcommand{\vec}{\operatorname{vec}}

\newcommand{\Proj}{\ensuremath{\mtx{\Pi}}} % Projection operator

%%% Semidefinite orders
\newcommand{\psdle}{\preccurlyeq}
\newcommand{\psdge}{\succcurlyeq}

\newcommand{\psdlt}{\prec}
\newcommand{\psdgt}{\succ}

%%% Mensuration: inner products and norms

% TeX does not like either \newcommand or \renewcommand for these
% two macros.  There is probably a good reason not to use them via
% \def, but I don't know it.  
%\newcommand{\<}{\langle} 
%\newcommand{\>}{\rangle}
\newcommand{\ip}[2]{\left\langle {#1},\ {#2} \right\rangle}
\newcommand{\absip}[2]{\abs{\ip{#1}{#2}}}
\newcommand{\abssqip}[2]{\abssq{\ip{#1}{#2}}}
\newcommand{\tworealip}[2]{2 \, \real{\ip{#1}{#2}}}

\newcommand{\norm}[1]{\left\Vert {#1} \right\Vert}
\newcommand{\normsq}[1]{\norm{#1}^2}

\newcommand{\lone}[1]{\norm{#1}_{\ell_1}}
\newcommand{\smlone}[1]{\|#1\|_{\ell_1}}
\newcommand{\linf}[1]{\norm{#1}_{\ell_\infty}}
\newcommand{\sone}[1]{\norm{#1}_{S_1}}
\newcommand{\snorm}[1]{\sone{#1}}
\DeclareMathOperator{\dist}{dist}

% Fixed-size inner products and norms are useful sometimes
\newcommand{\smip}[2]{\bigl\langle {#1}, \ {#2} \bigr\rangle}
\newcommand{\smabsip}[2]{\bigl\vert \smip{#1}{#2} \bigr\vert}
\newcommand{\smnorm}[2]{{\bigl\Vert {#2} \bigr\Vert}_{#1}}

% Specific norms that are used frequently
\newcommand{\enormdangle}{{\ell_2}}
\newcommand{\enorm}[1]{\norm{#1}}
\newcommand{\enormsm}[1]{\enorm{\smash{#1}}}

\newcommand{\enormsq}[1]{\enorm{#1}^2}

\newcommand{\fnorm}[1]{\norm{#1}_{\mathrm{F}}}
\newcommand{\fnormsq}[1]{\fnorm{#1}^2}

\newcommand{\pnorm}[2]{\norm{#2}_{#1}}
%\newcommand{\snorm}[1]{\norm{#1}_*}

\newcommand{\triplenorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

% Special cones
\newcommand{\Feas}{\mathcal{F}}
\newcommand{\Desc}{\mathcal{D}}
\newcommand{\NormC}{\mathcal{N}} % Normal cone
\newcommand{\sdim}{\delta}
\newcommand{\ddt}[1]{\dot{#1}}
\DeclareMathOperator{\Circ}{Circ}

\DeclareMathOperator{\Lip}{Lip}

\newcommand{\Lorentz}{\mathcal{L}}
\newcommand{\cC}{\mathcal{C}} % Set of nonempty, closed convex cones

\newcommand{\sgd}{\mathrm{D}} % acronym for SubGradient Distance

\newcommand{\sang}{\angle}


% MACROS ML

% \newcommand{\e}{\varepsilon}
\newcommand{\uniform}{\textsc{uniform}}
\newcommand{\rant}[1]{\textcolor{blue}{\textbf{[#1]}}}



% MACROS DA

\newcommand{\comm}[1]{\textcolor{OliveGreen}{[#1]}}
\newcommand{\IR}{\mathbbm{R}}
\newcommand{\veps}{\varepsilon}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\bface}{\overline{\mathcal{F}}}
\newcommand{\face}{\mathcal{F}}
\newcommand{\relint}{\operatorname{relint}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\Gr}{\operatorname{Gr}}
\newcommand{\powerset}{\mathscr{P}}
\newcommand{\hd}{{\operatorname{hd}}}
\newcommand{\inter}{{\operatorname{int}}}
\newcommand{\conv}{\operatorname{conv}}

% MACROS JAT

\newcommand{\minimize}{\text{minimize}\quad}
\newcommand{\subjto}{\quad\text{subject to}\quad}
\newcommand{\find}[1]{\text{Find }{#1}\quad\longrightarrow\quad}

\newcommand{\op}[1]{\mathsf{#1}}

% MACROS JNW

\newcommand{\E}{\Expect}

%================
% Convexity & duality
%================

\DeclareMathOperator{\discont}{discont}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\aTube}{\mathcal{T}_{s}}
\DeclareMathOperator{\distH}{\dist_{\mathcal{H}}}

\newcommand{\pInd}{\mathbb{1}} % Indicator function for probability

%\newcommand{\pInd}{\mathbf{1}} % Indicator function for probability
\newcommand{\cInd}{\mathfrak{i}} % Indicator function on a convex set

\newcommand{\dilation}{\mathscr{H}}

\newcommand{\Cat}{\mathrm{Cat}}

% \newcommand{\N}{\mathbbm{N}} %natural numbers
\newcommand{\Q}{\mathbbm{Q}} %rational numbers
%\newcommand{\bbS}{\mathbb{S}} %sphere \S is used for paragraph symbol
% \newcommand{\R}{\mathbbm{R}} %real numbers
\newcommand{\Rm}{\R^m}
\newcommand{\Rn}{\R^n}
\newcommand{\eR}{\overline{\R}} %extended real numbers
% \newcommand{\Z}{\mathbbm{Z}} %integers
\newcommand{\K}{\mathbbm{K}} %The field of scalars
% \newcommand{\C}{\mathbbm{C}} % complex numbers
\newcommand{\D}{\mathbbm{D}} % dense subset in field of scalars

\newcommand{\ind}{\mathbbm{1}} %indicatrix function
\newcommand{\II}{\mathbbm{1}}

\newcommand{\FL}[1]{(-\Delta)^{#1}}
\newcommand{\invHL}{(-\Delta)^{-\frac12}}
 
\newcommand{\tI}{\widetilde{I}}

\newcommand{\rbracket}[1]{\left(#1\right)}
\newcommand{\sbracket}[1]{\left[#1\right]}
\newcommand{\cbracket}[1]{\left\{#1\right\}}
% \newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\normp}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\seminormp}[2]{\left[ #1 \right]_{#2}}
% \newcommand{\abs}[1]{ \left| #1 \right|}
\newcommand{\innerp}[1]{\langle{#1}\rangle}
\newcommand{\dbinnerp}[1]{\langle\langle{#1}\rangle\rangle}
\newcommand{\vect}[1] {\pmb{#1}}
\newcommand{\mat}[1]{\pmb{#1}}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\Morrey}[2]{\widetilde{L}^{#1}(#2)}
\newcommand{\wMorrey}[2]{\widetilde{L}^{#1}_*(#2)}
\newcommand{\Campanato }[2]{\widetilde{\mathscr{L}}^{#1}(#2)}
\newcommand{\wCampanato }[2]{\widetilde{\mathscr{L}}^{#1}_*(#2)}
\newcommand{\pRieszP}[2]{\widetilde{I}_{#1}(#2)}
%===========================
% BLACK BOARD BOLD SYMBOLS
%===========================

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

% ====================
% CALLIGRAPHIC SYMBOLS
% ====================

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{ C}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}


\newcommand{\scrL}{\mathscr{L}}
%=====================
% BOLD FRAKTUR SYMBOLS
%=====================

\newcommand{\caA}{\boldsymbol{\frak A}}
\newcommand{\caB}{\boldsymbol{\frak B}}
\newcommand{\caC}{\boldsymbol{\frak C}}
\newcommand{\caD}{\boldsymbol{\frak D}}
\newcommand{\caE}{\boldsymbol{\frak E}}
\newcommand{\caF}{\boldsymbol{\frak F}}
\newcommand{\caG}{\boldsymbol{\frak G}}
\newcommand{\caH}{\boldsymbol{\frak H}}
\newcommand{\caI}{\boldsymbol{\frak I}}
\newcommand{\caJ}{\boldsymbol{\frak J}}
\newcommand{\caK}{\boldsymbol{\frak K}}
\newcommand{\caL}{\boldsymbol{\frak L}}
\newcommand{\caM}{\boldsymbol{\frak M}}
\newcommand{\caN}{\boldsymbol{\frak N}}
\newcommand{\caO}{\boldsymbol{\frak O}}
\newcommand{\caP}{\boldsymbol{\frak P}}
\newcommand{\caQ}{\boldsymbol{\frak Q}}
\newcommand{\caR}{\boldsymbol{\frak R}}
\newcommand{\caS}{\boldsymbol{\frak S}}
\newcommand{\caT}{\boldsymbol{\frak T}}
\newcommand{\caU}{\boldsymbol{\frak U}}
\newcommand{\caV}{\boldsymbol{\frak V}}
\newcommand{\caW}{\boldsymbol{\frak W}}
\newcommand{\caX}{\boldsymbol{\frak X}}
\newcommand{\caY}{\boldsymbol{\frak Y}}
\newcommand{\caZ}{\boldsymbol{\frak Z}}

%=====================
% FRAKTUR SYMBOLS
%=====================

\newcommand{\frA}{\frak A}
\newcommand{\frB}{\frak B}
\newcommand{\frC}{\frak C}
\newcommand{\frD}{\frak D}
\newcommand{\frE}{\frak E}
\newcommand{\frF}{\frak F}
\newcommand{\frG}{\frak G}
\newcommand{\frH}{\frak H}
\newcommand{\frI}{\frak I}
\newcommand{\frJ}{\frak J}
\newcommand{\frK}{\frak K}
\newcommand{\frL}{\frak L}
\newcommand{\frM}{\frak M}
\newcommand{\frN}{\frak N}
\newcommand{\frO}{\frak O}
\newcommand{\frP}{\frak P}
\newcommand{\frQ}{\frak Q}
\newcommand{\frR}{\frak R}
\newcommand{\frS}{\frak S}
\newcommand{\frT}{\frak T}
\newcommand{\frU}{\frak U}
\newcommand{\frV}{\frak V}
\newcommand{\frW}{\frak W}
\newcommand{\frX}{\frak X}
\newcommand{\frY}{\frak Y}
\newcommand{\frZ}{\frak Z}

% ==================
% SANS SERIF SYMBOLS
% ==================

\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfAb}{\mathsf{Ab}}
\newcommand{\sfAbc}{\mathsf{Ab_c}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfComp}{\mathsf{Comp}}
\newcommand{\sfCompp}{\mathsf{Comp}_2}
\newcommand{\sfInv}{\mathsf{Inv}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfModR}{\mathsf{Mod}_R}
\newcommand{\sfModZ}{\mathsf{Mod}_\Z}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfTop}{\mathsf{Top}}
\newcommand{\sfTopp}{\sfTop_2}

%===================
% GREEK BOLD SYMBOLS
%===================

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bchi}{\boldsymbol{\chi}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\boldeta}{\boldsymbol{\eta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\btheta}{\boldsymbol{\theta}^*}
\newcommand{\bTheta}{\boldsymbol{\Theta}}

%=============
% BOLD SYMBOLS
%=============

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bCH}{\mathbf{CH}} %space of charges
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bGL}{\mathbf{GL}} %grassmannian
\newcommand{\bH}{\mathbf{H}}
\newcommand{\obH}{\overline{\bH}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bdx}{\mathbf{dx}} % differential form
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}} 
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bdev}{\mathbf{dev}} %deviation
\newcommand{\bexc}{\mathbf{exc}} %spherical excess
\newcommand{\bExc}{\mathbf{Exc}} %Excess
\newcommand{\bRV}{\mathbf{RV}} %rectifiable varifolds

%===================
% MATH ROMAN SYMBOLS
%===================
\DeclareMathOperator{\arctanh}{\mathrm{arctanh}}
\DeclareMathOperator{\diam}{\mathrm{diam}}
\DeclareMathOperator{\rmadh}{\mathrm{adh}} %adh�rence
\DeclareMathOperator{\rmap}{\mathrm{ap}} %approximate limits and derivatives
\DeclareMathOperator{\rmBdry}{\mathrm{Bdry}} %boundary
\DeclareMathOperator{\rmcard}{\mathrm{card}} %cardinal
\DeclareMathOperator{\rmClos}{\mathrm{Clos}} %closure
\DeclareMathOperator{\rmCov}{\mathrm{Cov}} %covering
\DeclareMathOperator{\rmDer}{\mathrm{Der}} %derived functions
\DeclareMathOperator{\rmdiam}{\mathrm{diam}} %diameter
\DeclareMathOperator{\rmDiff}{\mathrm{Diff}}
\DeclareMathOperator{\rmdim}{\mathrm{dim}} %dimension
\DeclareMathOperator{\rmdist}{\mathrm{dist}} %distance
\DeclareMathOperator{\rmhdist}{\rmdist_{\mathscr{H}}} %Hausdorff distance
\DeclareMathOperator{\rmdiv}{\mathrm{div}} %divergence
\DeclareMathOperator{\rmextr}{\mathrm{extr}} %extreme points
\DeclareMathOperator{\rmfr}{\mathrm{fr}} %fronti�re
\DeclareMathOperator{\rmgen}{\mathrm{gen}}
\DeclareMathOperator{\rmgrad}{\mathrm{grad}} %gradient
\DeclareMathOperator{\rmgraph}{\mathrm{graph}} %graph
\DeclareMathOperator{\rmHess}{\mathrm{Hess}} %Hessian
\DeclareMathOperator{\rmHom}{\mathrm{Hom}} %homomorphisms
\DeclareMathOperator{\rmid}{\mathrm{id}} %the identity map
\DeclareMathOperator{\rmim}{\mathrm{im}} %image
\DeclareMathOperator{\rmint}{\mathrm{int}} %intérieur
\DeclareMathOperator{\rmInt}{\mathrm{Int}} %interior
\DeclareMathOperator{\rmLap}{\mathrm{Lap}} %Laplacian
\DeclareMathOperator{\rmlength}{\mathrm{length}}
\DeclareMathOperator{\rmLip}{\mathrm{Lip}} %Lipschitz constant
\DeclareMathOperator{\brmLip}{\mathbf{Lip}}
\DeclareMathOperator{\rmloc}{\mathrm{loc}}
\DeclareMathOperator{\rmosc}{\mathrm{osc}} %oscillation
\DeclareMathOperator{\rmProj}{\mathrm{Proj}} %projectors
\DeclareMathOperator{\rmset}{\mathrm{set}} %set
\DeclareMathOperator{\rmsign}{\mathrm{sign}} %sign
\DeclareMathOperator{\rmsing}{\mathrm{sing}} %singular set
\DeclareMathOperator{\rmsl}{\mathrm{slope}} %slope
\DeclareMathOperator{\rmspan}{\mathrm{span}} %span
\DeclareMathOperator{\rmspt}{\mathrm{spt}} %support
\DeclareMathOperator{\rmsupp}{\mathrm{supp}} %support, as well
\DeclareMathOperator{\rmTan}{\mathrm{Tan}} %tangent space or measure
\DeclareMathOperator{\rmtrace}{\mathrm{trace}} %trace
\renewcommand{\div}{\text{div}}

\DeclareMathOperator{\LHS}{LHS}
\DeclareMathOperator{\RHS}{RHS}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\nablaperp}{\nabla^\perp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\id}{id}
% \DeclareMathOperator{\Id}{\mathbb{I}}
\DeclareMathOperator*{\esssup}{ess\,sup}


\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmII}{\mathrm{II}}
\newcommand{\rmIII}{\mathrm{III}}
\newcommand{\rmIV}{\mathrm{IV}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmtI}{\mathrm{\widetilde{I}}}
\newcommand{\rmtII}{\mathrm{\widetilde{II}}}
\newcommand{\rmtIII}{\mathrm{\widetilde{III}}}
\newcommand{\rmtIV}{\mathrm{\widetilde{IV}}}
\newcommand{\rmtV}{\mathrm{\widetilde{V}}}

%================
% SPECIAL SYMBOLS
%================

\newcommand{\blseg}{\pmb{[}}
\newcommand{\brseg}{\pmb{]}}

%the following provide the P ... Q and ? ... X style used by D. Fremlin

\newcommand{\prf}{\negthinspace
\textbf{P}\negthickspace\negthickspace\negthinspace
\textbf{P}\negthickspace\negthickspace\negthinspace
\textbf{P}\thickspace }
\newcommand{\frp}{\negthinspace
\textbf{Q}\negthickspace\negthickspace\negmedspace
\textbf{Q}\negthickspace\negthickspace\negmedspace
\textbf{Q}\thickspace }
\newcommand{\quer}{\negthinspace
\textbf{?}\negthinspace\negthinspace\negthinspace
\textbf{?}\negthinspace\negthinspace\negthinspace
\textbf{?}\thickspace }
\newcommand{\reuq}{\negthinspace
\textbf{X}\negthickspace\negthickspace\negthickspace
\textbf{X}\negthickspace\negthickspace\negthickspace
\textbf{X}\thickspace }

%restriction of a measure by W.F. Pfeffer

\newcommand{\hel} {
\hskip2.5pt{\vrule height7pt width.5pt depth0pt}
\hskip-.2pt\vbox{\hrule height.5pt width7pt depth0pt}
\, }

\newcommand{\restr}{\hel}

%interior product, variant of the above

\newcommand{\leh} {
\hskip2.5pt\vbox{\hrule height.5pt width8pt depth0pt}
\hskip-.2pt{\vrule height8pt width.5pt depth0pt}
\, }

%the join of two currents
%WARNING: use within the displaystyle environment only

\newcommand{\cones} {
\times \negthickspace \negthickspace \negthickspace \times \medspace }

%simplexes a la Federer, left and right

\newcommand{\lseg}{\boldsymbol{[}\!\boldsymbol{[}}
\newcommand{\rseg}{\boldsymbol{]}\!\boldsymbol{]}}

%for use for terminating the proof of a claim

\newcommand{\cqfd} {
\renewcommand{\qedsymbol}{$\blacksquare$}
\qed
\renewcommand{\qedsymbol}{$\square$} }

%binomial coefficient

\newcommand{\bin}[2]{
\begin{pmatrix} #1 \\
#2 
\end{pmatrix}}

%dashed integrals

\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle
\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{%
\setbox0=\hbox{$#1{#2#3}{\int}$}
\vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}

% bold norms

\newcommand{\lno}{\left\bracevert}
\newcommand{\rno}{\right\bracevert}

% a symbol in the left margin

\newcommand{\hardone}{\marginpar{\flushright{$\maltese$}}}

% measure restriction
\newcommand{\mres}{\mathbin{\vrule height 1.6ex depth 0pt width
0.13ex\vrule height 0.13ex depth 0pt width 1.3ex}}

%==============
% ABBREVIATIONS
%==============

% \newcommand{\veps}{\varepsilon}
\newcommand{\bveps}{\boldsymbol{\veps}}
\newcommand{\vphi}{\varphi}
\newcommand{\wh}{\widehat}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

%=================
% RENEWCOMMANDS
%=================

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\subset}{\subseteq}
\renewcommand{\supset}{\supseteq}



%%%%%%%%%%%%%%

%\newcommand{\LL}{\mathop{\hbox{\vrule height 6pt width .5pt depth 0pt
%\vrule height .5pt width 3pt depth 0pt}}\nolimits}


%\newcommand{\res}{\mathop{\hbox{\vrule height 7pt width .5pt depth 0pt
%\vrule height .5pt width 6pt depth 0pt}}\nolimits}


\newcommand{\Om}{\Omega}
% \newcommand{\eps}{\varepsilon}
\newcommand{\tom}{\widetilde\Omega}
\newcommand{\e}{{\rm e}}
\newcommand{\de}{{\rm d}}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commands

%\newcommand{\ro}{\mathbb{R}}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\md}[1]{\left|#1 \right|}
\newcommand{\nrm}[1]{\left|\left| #1 \right|\right|}
\newcommand{\bct}[1]{\left(#1\right)}
\newcommand{\com}{\mathsf{c}}
\newcommand{\ds}[1]{\displaystyle{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\DD}{\mathbb{D}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\parf}{\partial_{x_1}}
\newcommand{\pars}{\partial_{x_2}}
\newcommand{\parff}{\partial_{x_1x_1}}
\newcommand{\parfs}{\partial_{x_1x_2}}
\newcommand{\parss}{\partial_{x_2x_2}}
\newcommand{\Div}{\nabla\cdot}
\newcommand{\Lap}{\Delta}
\newcommand{\Grad}{\nabla}
\newcommand{\Curl}{-\nabla^\perp\cdot}
\newcommand{\NLI}{(-\Delta)^{-1}}
\newcommand{\NLHI}{(-\Delta)^{-\frac12}}
\newcommand{\NLIalp}{(-\Delta)^{\alpha-1}}
\newcommand{\intRT}{\int_{\mathbb{R}^2}}
\newcommand{\HP}{\mathbb{R}^2_+}
\newcommand{\intHP}{\int_{\mathbb{bbR}^2_+}}

\newcommand{\pt}{\partial_t}
\newcommand{\ptau}{\partial_\tau}
\newcommand{\Kxy}{\frac{(x-y)^\perp}{|x-y|^{2+2\alpha}}}
\newcommand{\Kxby}{\frac{(x-\bar{y})^\perp}{|x-\bar{y}|^{2+2\alpha}}}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\tu}{\tilde{u}}
 \DeclareMathOperator{\tr}{tr}
 % \newcommand{\idiff}{\,\mathrm{d}}
% \newcommand{\diff}{\mathrm{d}}

\newcommand{\om}{\omega}
\newcommand{\tv}{\tilde{v}}
% \newcommand{\tu}{\tilde{u}}
% \newcommand{\la}{\langle}
% \newcommand{\ra}{\rangle} 
\newcommand{\T}{\bm{T}} 
\newcommand{\G}{\bm{G}} 
\newcommand{\Ra}{\bm{R}} 
% \newcommand{\D}{\mathbb{D}} 

\newcommand{\bmA}{\bm{A}}
\newcommand{\bmB}{\bm{B}}
\newcommand{\bmC}{\bm{C}}
\newcommand{\bmD}{\bm{D}}
\newcommand{\bmE}{\bm{E}}
\newcommand{\bmF}{\bm{F}}
\newcommand{\bmG}{\bm{G}}
\newcommand{\bmH}{\bm{H}}
\newcommand{\bmI}{\bm{I}}
\newcommand{\bmJ}{\bm{J}}
\newcommand{\bmK}{\bm{K}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmM}{\bm{M}}
\newcommand{\bmN}{\bm{N}}
\newcommand{\bmO}{\bm{O}}
\newcommand{\bmP}{\bm{P}}
\newcommand{\bmQ}{\bm{Q}}
\newcommand{\bmR}{\bm{R}}
\newcommand{\bmS}{\bm{S}}
\newcommand{\bmT}{\bm{T}}
\newcommand{\bmU}{\bm{U}}
\newcommand{\bmV}{\bm{V}}
\newcommand{\bmW}{\bm{W}}
\newcommand{\bmX}{\bm{X}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmZ}{\bm{Z}}

\newcommand{\bma}{\bm{a}}
\newcommand{\bmb}{\bm{b}}
\newcommand{\bmc}{\bm{c}}
\newcommand{\bmd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}} 
\newcommand{\bmg}{\bm{g}}
\newcommand{\bmh}{\bm{h}}
\newcommand{\bmi}{\bm{i}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmk}{\bm{k}}
\newcommand{\bml}{\bm{l}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bmn}{\bm{n}}
\newcommand{\bmo}{\bm{o}}
\newcommand{\bmp}{\bm{p}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmr}{\bm{r}}
\newcommand{\bms}{\bm{s}}
\newcommand{\bmt}{\bm{t}}
\newcommand{\bmuslant}{\bm{u}}
\newcommand{\bmv}{\bm{v}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmy}{\bm{y}}
\newcommand{\bmz}{\bm{z}}

% Please don't change the following lines without a good reason -Mike
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "final"
%%% End:
